Vacuum-Bounded States and the Entropy of Black Hole Evaporation

We call a state ``vacuum bounded'' if every measurement performed outside a specified interior region gives the same result as in the vacuum. We compute the maximum entropy of a vacuum-bounded state with a given energy for a one-dimensional model, with the aid of numerical calculations on a lattice. For large energies we show that a vacuum-bounded system with length $L_in$ and a given energy has entropy no more than $S^rb + (1/6) \ln S^rb$, where $S^rb$ is the entropy in a rigid box with the same size and energy. Assuming that the state resulting from the evaporation of a black hole is similar to a vacuum-bounded state, and that the similarity between vacuum-bounded and rigid box problems extends from 1 to 3 dimensions, we apply these results to the black hole information paradox. Under these assumptions we conclude that large amounts of information cannot be emitted in the final explosion of a black hole. We also consider vacuum-bounded states at very low energies and come to the surprising conclusion that the entropy of such a state can be much higher than that of a rigid box state with the same energy. For a fixed $E$ we let $L_in'$ be the length of a rigid box which gives the same entropy as a vacuum-bounded state of length $L_in$. In the $E\to 0$ limit we conjecture that the ratio $L_in'/L_in$ grows without bound and support this conjecture with numerical computations.

==> defs.tex <==
% Definitions
\makeatletter

% Miscellaneous definitions
%\def\mynote#1{\footnote{\sf #1}}

\def\qed{\hspace{.3em}\rule[-.1ex]{.4em}{2ex}} % Black block
% This is a hacked up version of \copyright
\def\trademark{\raise .5ex\hbox{\ooalign{\hfil\raise.07ex\hbox{\scriptsize
R}\hfil\crcr\mathhexbox20D}}}

% Inverse transpose as a single superscript
\def\invt{{{-1}^{\scriptstyle T}}}

% A version of \delta for use in variations of quantities.  It comes closer
% to the quantity that is varied.
\def\ddelta{\delta\hskip -.07em}

% Not-summed symbol.  Because of the nature of a sigma the slash looks
% a bit better further to the right.
\newbox\sumbox
\setbox\sumbox=\hbox{$\sum$}
\def\notsum{\hbox to 0pt{\hskip .6\wd\sumbox minus 1 fil\mbox{\Large /}%
\hskip -.6\wd\sumbox minus 1 fil}\copy\sumbox}

% Equation environments
% Here is a variant eqnarray environment that doesn't have stupid
% extra space around the = signs.
\newenvironment{neqnarray}{\begingroup\arraycolsep 2pt\begin{eqnarray}}{\end{eqnarray}\endgroup}

% \be = \begin{equation}. 
% \be[name] = \begin{equation}\label{eqn:name}
% \ee = \end{equation}
\def\be{\@ifnextchar[{\be@label}{\begin{equation}}} % ]
\def\be@label[#1]{\begin{equation}\label{eqn:#1}}
\def\ee{\end{equation}}

% \bea begins an equation array.  Syntax as above.  This is what you
% want when you are breaking an equation over several lines.
\def\bea{\@ifnextchar[{\bea@label}{\begin{neqnarray}}} % ]
\def\bea@label[#1]{\begin{neqnarray}\label{eqn:#1}}
\def\eea{\end{neqnarray}}

% \blea begins an equation array with letters.  This is what you want
% when you have several equations.
\def\blea{\@ifnextchar[{\blea@label}{\begin{mathletters}\begin{neqnarray}}} %]
\def\blea@label[#1]{\begin{mathletters}\label{eqn:#1}\begin{neqnarray}}
\def\elea{\end{neqnarray}\end{mathletters}}

% References to equations, etc.

\def\eqref#1{Eq.\ (\ref{eqn:#1})}
\def\eqsref#1{Eqs.\ (\ref{eqn:#1})} % If more than one use \ref
\def\Eqref#1{Equation (\ref{eqn:#1})}	% For starting sentence
\def\Eqsref#1{Equations (\ref{eqn:#1})}
\def\figref#1{Fig.\ \ref{fig:#1}}
\def\figsref#1{Figs.\ \ref{fig:#1}} % You have to supply the rest yourself
\def\lemref#1{lemma \ref{lem:#1}}
\def\secref#1{section \ref{sec:#1}}
\def\thmref#1{theorem \ref{thm:#1}}

% Math operators

\let\member=\in
\def\csch{\text{csch}\,}
\def\<{\langle }
\def\>{\rangle }
\def\Tr{\text{Tr}\,}
\def\Trin{\text{Tr}_\in\,}
\def\diag{\mathop{\rm diag}}

% Combinations of matrix parts for convenient use in subscripts
\def\freefree{{\text{free},\text{free}}}
\def\freegs{{\text{free},\text{gs}}}
\def\freeout{{\text{free},\text{out}}}
\def\freein{{\text{free},\text{in}}}
\def\gsfree{{\text{gs},\text{free}}}
\def\gsgs{{\text{gs},\text{gs}}}
\def\gsout{{\text{gs},\text{out}}}
\def\gsin{{\text{gs},\text{in}}}
\def\outfree{{\text{out},\text{free}}}
\def\outgs{{\text{out},\text{gs}}}
\def\outout{{\text{out},\text{out}}}
\def\outin{{\text{out},\text{in}}}
\def\infree{{\text{in},\text{free}}}
\def\ings{{\text{in},\text{gs}}}
\def\inout{{\text{in},\text{out}}}
\def\inin{{\text{in},\text{in}}}
\def\midmid{{\text{mid},\text{mid}}}
\def\inmid{{\text{in},\text{mid}}}

% Theorem-like structures
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
% Don't number definitions, because there is only one.
\def\thedefinition{\unskip}	% Unskip removes space added before number

% Misc

\def\half{{1\over 2}}
\def\qtr{{1\over 4}}


% Typeset matrices split up into blocks

% Matrix zero except in lower left.
\def\lowerleftnonzero#1{\arraycolsep 0pt
% This removes vertical space between the lines and the -g
\renewcommand\arraystretch{0}
\left(\begin{array}{cc}
\noalign{\vspace{1ex}}
& \hspace{1em} 0 \hspace{1em} \\
\noalign{\vspace{1ex}}
\cline{1-1}
#1 \hspace{2pt} & \vline \hfill
\end{array}\right)}


%% Matrix split into two block columns
\def\joinmatrix(#1,#2){
\left(\begin{array}{c|c}
   #1 & #2
   \end{array}\right)}

% Split into block columns and give sizes.  
% 1 and 2 are elements, 3, 4 widths, 5 height
% See comments in sizedsplitmatrix
\def\sizedjoinmatrix(#1,#2)(#3,#4)(#5){
\left(\begin{array}{c|c}
	\noalign{\global\setbox\myarstrut=\box\@arstrutbox} % Move strut
	\matrixwidth{#3} & \matrixwidth{#4} \\ % Header line
	 \copy\myarstrut #1 & #2 \\
	\end{array}\right)
% Tell Tex about actual height
\vrule width 0pt height 2\ht\myarstrut
\} \scriptstyle #5
}

%% Matrix split into row blocks
\def\stackmatrix(#1,#2){
{\renewcommand\arraystretch{1.1}
\left(\begin{array}{c}
	#1 \\ \hline #2
	\end{array}\right)}}

%% Split into blocks with heights.  See sizedsplitmatrix.
\def\sizedstackmatrix(#1,#2)(#3)(#4,#5){
{\renewcommand\arraystretch{1.1}
\left(\begin{array}{c}
	\noalign{\global\setbox\myarstrut=\box\@arstrutbox} % Move strut
	\matrixwidth{#3} \\ % Header
	\copy\myarstrut #1 \\ \hline
	\copy\myarstrut #2
	\end{array}\right)
\vrule width 0pt height 3\ht\myarstrut
\hspace{-4pt}
\begin{array}{l}	% Labels to right of array
   \}\scriptstyle #3 \\
   \}\scriptstyle #4
\end{array}}}

%% Typeset a matrix made of 4 blocks.
\def\splitmatrix(#1,#2,#3,#4){
{\renewcommand\arraystretch{1.1} % Keep superscript from colliding with line
\left(\begin{array}{c|c}
	#1 & #2 \\ \hline
	#3 & #4
	\end{array}\right)
}}

\newbox\ulstrut
\savebox{\ulstrut}{\vrule width 0pt depth 10pt height 15pt}

%% Case where upper left is one number but rest is larger
\def\splitmatrixul(#1,#2,#3,#4){
{\renewcommand\arraystretch{1.1} % Keep superscript from colliding with line
\arraycolsep 2pt
\left(\begin{array}{c|@{\hspace{10pt}}c@{\hspace{10pt}}}
	#1 & #2 \\ \hline
	\copy\ulstrut #3 & #4
	\end{array}\right)
}}



%% Typeset a matrix made of 4 blocks and label the height and the
%% width.  Here's how it works:
%%    Latex uses a strut in @arstrutbox to make the lines of the array
%%    the right height.  We remove it and put it in myarstrut.  Then
%%    we set an extra, zero-height row at the top of the matrix which
%%    holds the width labels above it.  Then we explicitly use the
%%    strut to make the row the right size.  Because now Tex doesn't 
%%    know about the stuff that sticks up we make a strut to keep it from
%%    hitting stuff above it.

%% This is conditionalized to allow the upper left element to be smaller
%% than the rest.

\newbox\myarstrut
\newif\ifmatrixul		% Makes upper left smaller
\newlength{\myextrastrutlength}

% 1,2,3,4 are actual elements, 5,6 are widths and 7,8 are heights
\def\sizedsplitmatrix(#1,#2,#3,#4)(#5,#6)(#7,#8){
{\renewcommand\arraystretch{1.1} % Keep superscripts from colliding
\ifmatrixul\arraycolsep 2pt\fi
\left(\begin{array}{c|\ifmatrixul @{\hspace{10pt}}c@{\hspace{10pt}}
		      \else c \fi}
	\noalign{\global\setbox\myarstrut=\box\@arstrutbox} % Move strut
	\matrixwidth{#5} & \matrixwidth{#6} \\ % Header line
	 \copy\myarstrut #1 & #2 \\ \hline
	 \ifmatrixul \copy\ulstrut \else \copy\myarstrut \fi #3 & #4
	\end{array}\right)
}
% Tell Tex about actual height
\ifmatrixul
\setlength{\myextrastrutlength}{2\ht\myarstrut}
\addtolength{\myextrastrutlength}{\ht\ulstrut}
\vrule width 0pt height \myextrastrutlength
\else
\vrule width 0pt height 3\ht\myarstrut
\fi
\hspace{-4pt}
\begin{array}{l}	% Labels to right of array
   \}\scriptstyle #7 \\
   \ifmatrixul\copy\ulstrut\bigg\}\else\}\fi\scriptstyle #8
\end{array}
}

% Make a box of zero height and width which anchors a label above it
\def\matrixwidth#1{
  \vbox to 0pt{\vskip 0pt minus 1fil%    Skip back up to top of label
    \hbox{$\scriptstyle #1$}\vskip 2pt}}

% Typeset with upper left element smaller
\def\sizedsplitmatrixul(#1,#2,#3,#4)(#5,#6)(#7,#8){
{\matrixultrue\sizedsplitmatrix(#1,#2,#3,#4)(#5,#6)(#7,#8)}}



% Figures

% \mypsfig{LABEL}{CAPTION} produces an epsf figure at the current
% place from the file LABEL.ps and tags it with LABEL.
\def\mypsfig#1#2{%
\begin{figure}
\begin{center}
\vspace{-1ex}
\leavevmode\epsfbox{#1.ps}
\vspace{-1.7ex}
\end{center}
\caption{#2}
\label{fig:#1}
\end{figure}}

% Same but offset figure to left to compensate for missing axis label
\def\mypsfigoff#1#2{%
\begin{figure}
\begin{center}
\vspace{-1ex}
\leavevmode\hskip -15pt\epsfbox{#1.ps}
\vspace{-1.7ex}
\end{center}
\caption{#2}
\label{fig:#1}
\end{figure}}



% \mypsfigr{LABEL}{CAPTION}.  Does mypsfig and  and refers to it
% with figref.
\def\mypsfigr#1#2{\mypsfig{#1}{#2}\figref{#1}}

\def\mypsfigroff#1#2{\mypsfigoff{#1}{#2}\figref{#1}}

% \mypsfigloc{LABEL}{CAPTION}{LOC} give LOC argument to figure env.
% \def\mypsfigloc#1#2#3{%
% \begin{figure}[#3]
% \begin{center}
% \vspace{-1ex}
% \leavevmode\epsfbox{#1.ps}
% \vspace{-1ex}
% \end{center}
% \caption{#2}
% \label{fig:@cap#1}
% \end{figure}}


% Cram floats together
\floatsep 0pt

% Make captions narrower, and append period to caption that is set, but
% not one in list of figuers

\newlength{\captionsize}
\setlength{\captionsize}{.8\textwidth}

\long\def\@makecaption#1#2{
\vskip 10pt			% Space after figure
\setbox\@tempboxa\hbox{\sl #1: #2.}	% Try typesetting caption on one line
\hbox to\hsize{\hfil		% Center it
\ifdim \wd\@tempboxa >\captionsize	% Bigger than one line?
\parbox{\captionsize}{\sl #1: #2.}	% Yes: Set in parbox
\else\box\@tempboxa		% No, just use it.
\fi
\hfil}}

% Notation system 
% Flag for actually producing the notation page.
\newif\ifsetnotation

% \notationx{TAG}{NOTATION}{DESCRIPTION} sets a notation line and
% defines a macro \@notationlabelTAG to mark that tag was used.  The
% first such use will be the page number that appears in the list.
% Tag is something arbitrary used for labeling.
% \@dottedtocline is more complex than we need, but it does the job.
\def\notationx#1#2#3{%
\ifsetnotation			% Second pass -- set notation page
\@dottedtocline{1}{0em}{2em}{\mynumberline{#2} --- #3}{\pageref{not:#1}}
\else
\global\@namedef{notationlabel@#1}{%	First pass.  Define label macro:
\ifsetnotation			% If still on notation page, don't
%				% label here
\else				%
\label{not:#1}%				Mark current page of use.
\global\@namedef{notationlabel@#1}{}%	And redefine itself to do nothing
\@addckptnotation{#1}%			And remember this in checkpoint
\fi}				% End of label macro definition
\fi
}

% This is like numberline, except that if the item is too wide
% it just pushes the rest of the line over.
\def\mynumberline#1{\setbox\@tempboxa\hbox{#1}% Look at size
\ifdim \wd\@tempboxa > \@tempdima % Does it fit
\box\@tempboxa			% No, just set it
\else
\hbox to\@tempdima{#1\hfil}%	Yes, do indentation after
\fi}

% \notationlabel{TAG} labels that this is the place where the notation
% specified by TAG is used.  Only the first page appears in the list.
% Uses on the notation page itself are not labelled.
\def\notationlabel#1{\@nameuse{notationlabel@#1}}

% In the usual case we use the same thing for the tag and the notation
\def\notation#1#2{\notationx{#1}{$#1$}{#2}}
\def\usenotation#1{$#1$\notationlabel{#1}}

% \defnotationx{MACRO}{NOTATION}{NOTATION-FOR-LIST}{DESCRIPTION}
% set a notation line here using NOTATION-FOR-LIST and DESCRIPTION and
% defines \MACRO to expand into NOTATION and label first use.
\def\defnotationx#1#2#3#4{%
\notationx{#1}{#3}{#4}%		Emit notation line now.
\global\@namedef{#1}{#2\notationlabel{#1}}} % Define to use code and mark

% The above macro puts the object first, and then does the label.  Now
% labels, in order to get the page number right, work by putting a whatsit
% box in the current list, and only writing the aux file later when the page
% number is known.  Thus you have to deal with keeping this extra thing
% out of your way.  There are three places it can go:
%  \defnotationx puts it after the item.  This is good when there is a \bar
%	or something like that first.  It doesn't work with subscripts.
%  \defnotationsubx puts it before the item.  This allows your item to
%       have subscripts, but not \bar.
%  \defnotationgrpx puts a group around your item and the extra box.  This
%	is good when your item IS a subscript or the like.  It doesn't
%	work well when your item has subscripts.

\def\defnotationsubx#1#2#3#4{%
\notationx{#1}{#3}{#4}%		Emit notation line now.
\global\@namedef{#1}{\notationlabel{#1}#2}} % Define to use code and mark

\def\defnotationgrpx#1#2#3#4{%
\notationx{#1}{#3}{#4}%		Emit notation line now.
\global\@namedef{#1}{{\notationlabel{#1}#2}}} % Define to use code and mark

% The usual case has the expansion appearing in the notation list.
\def\defnotation#1#2#3{\defnotationx{#1}{#2}{$#2$}{#3}}
\def\defnotationsub#1#2#3{\defnotationsubx{#1}{#2}{$#2$}{#3}}
\def\defnotationgrp#1#2#3{\defnotationgrpx{#1}{#2}{$#2$}{#3}}

% Interaction with checkpoint system
\def\@ckptnotation{}		% List of notations to checkpoint
\def\@addckptnotation#1{\@cons\@ckptnotation{{#1}}}

% This extends a system definition
\def\@writeckpt#1{\if@filesw 
\immediate\write\@partaux{\string\global\string\@namedef{cp@#1}\@charlb}% 
{\let\@elt\@wckptelt \cl@@ckpt}%
{\let\@elt\@wckptnotationelt \@ckptnotation}%  New code to write notations
\immediate\write\@partaux{\@charrb}%
\fi}

% Write out forms to define the notationlabel macros not to do anything
\def\@wckptnotationelt#1{\immediate\write\@partaux
{\string\global\string\@namedef{notationlabel@#1}{}}}


\makeatother

